On the Existence of Information Bottlenecks in Living and Non-Living Systems

In many complex systems, we observe that `interesting behaviour' is often the consequence of a system exploiting the existence of an Information Bottleneck (IB). These bottlenecks can occur at different scales, between individuals or components of a system, and sometimes within individuals themselves. Oftentimes, we regard these bottlenecks negatively; as merely the limitations of the individual's physiology and something that ought to be overcome when designing and implementing artificial systems. However, we suggest instead that IBs may serve a purpose beyond merely providing a minimally-viable channel for coordination in collective systems. More specifically, we suggest that interesting or novel behaviour occurs when the individuals in a system are constrained or limited in their ability to share information and must discover novel ways to exploit existing mechanisms, which are inherently bottlenecked, rather than circumventing or otherwise avoiding those mechanisms entirely.

==> sections/communication_protocols.tex <==
Information transferred through bottlenecks must follow \textit{protocols} to be comprehended by receivers. 

Human individuals understand sound (voice) or visual (writing) stigmagies made by others as long as they follow forms of languages. Similarly, digital signals exchanged on the internet must follow certain protocols to be comprehended by devices. In both cases, bottlenecked information transfer follow certain protocols of communication. In the case of human language communication, languages are obtained through education as if web engineers learn communicatoin protocols. 

TO DO: definition of protocols; origin of protocols; examples of protocols; 

==> sections/decoder_encoder_framework.tex <==
As we have discussed so far, the bottlenecks exist among communicating agents because it is essentially impossible to copy and paste one's experiences, thoughts or internal representations to others. Thus, information passed from a sender to a receiver has to take different forms from what in the sender's mind. For instance, in the case of ants' pheromones described above, the pheromones is not exactly what ants observed. However, the secreted pheromones are interpreted by other individuals and transmitted to further members of a colony. Thus, communicating agents through information bottlenecks must interpret implicit contents from codes that has passed the bottlenecks. In other words, communication among agents through bottlenecks can be seen as decoding contents from codes that are informatically reduced from original contents. Also, regardless that the reduction of content to codes is conducted intentionally and unintentionally, this information processing that senders are taking accounts can be considered as encoding of contents to reduced codes. Thus, the communication through bottlenecks is, to some extent, an encoding-decoding process of contents. 

This type of information processing can be seen in well-known autoencoder models in artificial neural networks. These computational models encode high dimensional inputs to low dimensional forms in a latent space and decode the low dimensional forms to high dimensional outputs. Although the autoencoders' encoding process is usually considered as abstraction, the encodings in both autoencoders and information bottlenecks reduce dimensions or complexity from raw contents, and there ain't not huge gaps between them. 
The largest difference between bottlenecked communications and autoencoders is that encoders and decoders are different individuals in the former while the latter is within an individual. Also, in cases of collective systems like ant colonies, individuals which decode and encode information are connected like chains of decoder-encoder and information is shared among a population. Therefore, collective systems communicating through information bottlenecks can be represented as multi-decoder-encoder systems. 


==> sections/information_domains.tex <==
This section explores how bottlenecks arise from systems naturally along with individuality and collectiveness. To some extent, information, or some more generalized forms of it, must be passed from one (sender) to others (receivers) and makes a change on the receivers regardless of its scale. Also, informatoin bottlenecks, by definition, occur between a sender and a receiver. Our intuition is bottlenecks always exist if information is transferred between what we call individuated information domains. Informatoin domains are domains in spatio-temporal field that are bounded by barriers on information transfer. In other words, an information domains is a domain outside of which information is not completely exchanged with inside. 

An example case that information domains can appear is group of people talking in a noisy place. In an environment where is full of noisy sounds, people talking have to be close to each other (even if they can speak loudly, the range of voice transmitting is limited in some distance). In this case, the area in which people can talk without loss of hearable voice is information domain, and once someone walks out from this area, the person will experince loss of informatoin spoken from somebody in the area. 

Another exmaple of informatoin domain is radio broadcasting. In FM broadcasting, radio channels in a region differentiate their signals by using unique frequency bands so that their signals do not mixed with others (here, bands correspond to informaotin domains in the exmaple above). However, this differentiation works only in a limited region because signals are mixed with other regional channels that use same frequency band in border zones (this does not happen in most of real world because channels use different bands from channels in neighbouring regions). In this case, the zones of signal mixtures bound zones of proper signal transferring into domains in which information can be transferred without comtaminations with others. These domains correspond to domains in more macroscopic levels than the first exmaple. 

These information domains bounded by noisy zones can enjoy complete information transferring within domains. However, there are difficulties when domains intercommunicate because information emitted from a domain is comtaminated or totally replaced with noises. One way to overcome this problem is building communication pipelines that allow domains to exhange information with anti-noise protections. However, these pipelines are still limited in terms of quality and quantity. Otherwise, if these pipelines are unlimited and information is completely transferred among domains, these domains are a single domain by definition. Here, the limitions on inter-domain information transfer is the information bottlenecks as exmaples given earlier (next section examines how inter-domain communication with bottlenecks can take account in collective systems by introducing the concept of \textit{protocol}). In other words, information bottlenecks are inevitable byproducts of individuation of information domains. Although this paper will not go deeply into the concept of individuality, it is possible to position systems on a range of individuation of information domains with information bottlenecks and noisy boundaries; \textit{continuous}, \textit{smooth}, \textit{discrete} systems. 

Continuous systems are systems without boundaries or bottlenecks expect locational bottleneck. This kind of systems are made of points, or an entire system is a continuous surface or volume. All points of the surface receive information from neighbouring area without any losses. Continuous systems are on what other kinds of systems to occur. Examples of continuous systems can be electromagnetic fields. Smooth Life and Lenia are, in theory, continuous systems. 

Smooth systems are systems without bottlenecks expect locational bottleneck. Smooth systems are made of particles or grids, or more generally, separated domains from each other but they exchange information without  any losses. In other words, smooth systems are made of separated domains that receive and send information that is completely same as other domains’ states (or complete information to describe other domains). For example, Most of cellular automata, such as Conway’s game of life, are made of multiple cells (which are considered as particles) which are described by states (alive/dead and position) and receive complete information of neighbouring cells’ states (alive/dead and position) to update their states. Reynolds' Boid model is also smooth because each agent receives neighbouring agents’ states (velocity and position). In general, all of modern day computable systems are smooth systems are higher rank.

Discrete systems are systems with bottlenecks. Discrete systems are made of separated domains that are bounded and cannot exchange complete states that describe domains. 
